Rethinking Backdoor Adversarial Unlearning through the Lens of Catastrophic Forgetting in Continual Learning

Existing studies reveal that current backdoor defenses exhibit limited robustness and often fail against specific types of attacks. More concerningly, prevailing safety tuning strategies tend to provide only superficial safety protection, as they fall short of completely eliminating the backdoor effects. In this work, we present a novel formulation of backdoor learning and unlearning as a sequential, three-stage process from a continual learning perspective. Within this framework, we formally define complete backdoor unlearning and further derive the necessary conditions for achieving it based on the mechanism of catastrophic forgetting. Guided by these insights, we propose Blind Inversion-Backdoor Adversarial Unlearning (BI-BAU), which formulates the generation of adversarial examples satisfying the unlearning conditions as a blind inversion problem. We solve this by integrating the bi-level optimization process of adversarial training into an Expectation-Maximization (EM) algorithm framework to optimize the maximum a posteriori (MAP) objective. Furthermore, BI-BAU is extended to untargeted adversarial scenarios with unknown target classes, as well as to multi-modal contrastive learning tasks, enhancing its applicability to real-world deployment scenarios where pre-trained models may be compromised. Extensive experiments demonstrate that our method exhibits general applicability across a wide spectrum of backdoor attacks and can effectively and thoroughly eliminate the backdoor effects from a backdoor model.

==> section/Abstract.tex <==
%%%%%%%%% ABSTRACT
\begin{abstract}
Existing studies reveal that current backdoor defenses exhibit limited robustness and often fail against specific types of attacks. More concerningly, 
prevailing safety tuning strategies tend to provide only superficial safety protection, as they fall short of completely eliminating the backdoor effects.
In this paper, we are the first to formulate the process of backdoor learning and unlearning as a sequential three-stage supervised learning task within 
a continual learning framework. Within this framework, we formally define complete backdoor unlearning and futher derive the necessary conditions for achieving it
through a theoretical analysis grounded in the catastrophic forgetting mechanism. Based on this foundation, we propose Blind Inversion-Backdoor Adversarial Unlearning (BI-BAU), 
which reformulates the generation of adversarial examples that satisfy the complete unlearning conditions as a blind inversion problem.
We solve this by integrating the bi-level optimization process of adversarial training into an Expectation-Maximization (EM) algorithm framework to optimize 
the maximum a posteriori (MAP) objective. Extensive experiments demonstrate that our method exhibits general applicability across a large spectrum of backdoor attacks, 
and can effectively and thoroughly eliminate the backdoor effects from a backdoor model.
\end{abstract}

% \begin{abstract}
%     Existing studies indicate that current backdoor defense methods often exhibit limited robustness and remain vulnerable to attacks 
%     with low orthogonality or low linearity.
%     More concerningly, current safety tuning strategies may offer only superficial safety protection, as they fail to completely eliminate the backdoor effects embedded 
%     within compromised models.
%     In this paper, we are the first to formulate the process of backdoor learning and unlearning as a sequential three-stage supervised learning task within a continual learning framework, 
%     in order to explore the core challenges of backdoor unlearning. 
%     Building upon a theoretical analysis grounded in the mechanism of catastrophic forgetting, we introduce the novel concept of complete backdoor unlearning 
%     and provide a formal definition, along with the necessary conditions for achieving it.
%     Based on this foundation, we propose Blind Inversion–Backdoor Adversarial Unlearning (BI-BAU), which reformulates the construction of condition-satisfying 
%     adversarial examples as a Blind Inversion problem and solve this by integrating the bi-level optimization process of adversarial training into an Expectation-Maximization (EM) 
%     algorithm framework to optimize the $\text{MAP}_{\theta}$ objective.
%     Extensive experiments demonstrate that our method exhibits general applicability across a wide range of backdoor threats, 
%     and can effectively and thoroughly eliminate the backdoor effects from compromised models.
% \end{abstract}



% 1. 清晰地阐明当前研究的问题 ---> 
% 2. 我们的工作介绍 ---> 
% (四大块递进清晰:Problem Formulation, Complete Backdoor Unlearning, Blind Inversion, Proposed method )
% 3. 效果说明


% 当前研究现状：

% Despite the promising progress achieved by existing works on safety tuning, they inevitably suffer from several limitations, such as the need to train additional 
% models for synthesizing backdoor triggers, resulting in high computational costs, constraints imposed by underlying assumptions that affect their applicability, 
% and a lack of rigorous theoretical grounding, which makes it difficult to ensure robustness. 

% Moreover, Zhang~\etal~\cite{zhang2024exploring} conduct a comprehensive analysis of mainstream backdoor attacks and defenses, revealing that existing defense mechanisms 
% are particularly susceptible to attacks characterized by low orthogonality or low linearity. More concerningly, recent studies~\cite{zhu2024breaking,min2024uncovering} 
% reveal that current defense methods may provide only superficial safety, as they fail to eliminate the backdoor effects embedded in compromised models completely. 

% As a result, adversaries can still easily reactivate the implanted backdoor by exploiting residual backdoor features that persist within the purified model. 
% As illustrated by the Retuning Attack proposed by Min~\etal~\cite{min2024uncovering}, a backdoor can be effectively reactivated by fine-tuning a purified model 
% for a few epochs using a dataset that contains only a small portion of poisoned samples. 


% 我们的工作。

% To the best of our knowledge, we are the first to theoretically explore the core challenges of backdoor unlearning from the perspective of continual learning. 
% In addition, we provide a formal definition of complete backdoor unlearning. Through a theoretical analysis grounded in catastrophic forgetting mechanism, 
% we further establish the necessary condition that the backdoor unlearning task must fulfill to achieve the object of complete backdoor unlearning.

% Building on the necessary condition for achieving complete backdoor unlearning, we propose Blind Inversion-Backdoor Adversarial Unlearning (BI-BAU). 
% This method reformulates the construction of adversarial examples that satisfy the condition as a Blind Inversion problem. By integrating the bi-level optimization 
% process of adversarial training into the Expectation-Maximization (EM) algorithm framework to optimize the MAPθ objective, our
% method effectively and thoroughly eliminates the backdoor effects from the compromised model.


% We conduct a comprehensive investigation of existing backdoor attack methods. Extensive experiments demonstrate that our method exhibits general appli-
% cability against a wide range of backdoor threats, including more challenging cases such as attacks with low orthogonality or low linearity [23]. Moreover, 
% it achieves a truly complete removal of backdoor effects.



